Formalizing Factorization on Euclidean Domains and Abstract Euclidean Algorithms

This paper discusses the extension of the Prototype Verification System (PVS) sub-theory for rings, part of the PVS algebra theory, with theorems related to the division algorithm for Euclidean rings and Unique Factorization Domains that are general structures where an analog of the Fundamental Theorem of Arithmetic holds. First, we formalize the general abstract notions of divisibility, prime, and irreducible elements in commutative rings, essential to deal with unique factorization domains. Then, we formalize the landmark theorem, establishing that every principal ideal domain is a unique factorization domain. Finally, we specify the theory of Euclidean domains and formally verify that the rings of integers, the Gaussian integers, and arbitrary fields are Euclidean domains. To highlight the benefits of such a general abstract discipline of formalization, we specify a Euclidean gcd algorithm for Euclidean domains and formalize its correctness. Also, we show how this correctness is inherited under adequate parameterizations for the structures of integers and Gaussian integers.

==> eptcsdata.tex <==
\providecommand{\firstpage}{18}
\providecommand{\publicationstatus}{Temur Kutsia, Daniel Ventura, David Monniaux \&\\
 Jos\'e F. Morales (Eds.): LSFA 2023 + HCVS 2023\\
EPTCS 402, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.402.5}{10.4204/EPTCS.402.5}}
\pdfoutput=1

